MHLA: Restoring Expressivity of Linear Attention via Token-Level Multi-Head

While the Transformer architecture dominates many fields, its quadratic self-attention complexity hinders its use in large-scale applications. Linear attention offers an efficient alternative, but its direct application often degrades performance, with existing fixes typically re-introducing computational overhead through extra modules (e.g., depthwise separable convolution) that defeat the original purpose. In this work, we identify a key failure mode in these methods: global context collapse, where the model loses representational diversity. To address this, we propose Multi-Head Linear Attention (MHLA), which preserves this diversity by computing attention within divided heads along the token dimension. We prove that MHLA maintains linear complexity while recovering much of the expressive power of softmax attention, and verify its effectiveness across multiple domains, achieving a 3.6\% improvement on ImageNet classification, a 6.3\% gain on NLP, a 12.6\% improvement on image generation, and a 41\% enhancement on video generation under the same time complexity.

==> tabs/tab_dataset_statics.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{\textbf{Comparison of representative robotic video datasets.}}
\resizebox{\textwidth}{!}{

\begin{tabular}{lcccccccc}
\toprule
\textbf{Dataset} & \textbf{Year} & \textbf{\#Videos} & \textbf{\#Skills}  & \textbf{Resolution} & \textbf{Optical Flow} & \textbf{Diverse Robotic Forms} & \textbf{Diverse Captions} \\
\midrule
RoboTurk~\cite{mandlekar2018roboturk}            & 2018  & 2.1k  & 2 & 480P & \xmark  & \xmark & \xmark \\
RoboNet~\cite{dasari2019robonet}                 & 2019  & 162k & N/A & 240P & \xmark  & \xmark & \xmark \\
BridgeData~\cite{ebert2021bridge}                & 2021  & 7.2k & 4 & 480P & \xmark  & \xmark & \xmark \\
RH20T~\cite{fang2023rh20t}                       & 2023  & 13k & 33 & 720P & \xmark  & \xmark & \xmark \\
DROID~\cite{khazatsky2024droid}                  & 2024  & 76k & 86 & 720P & \xmark  & \xmark & \xmark \\
Open X-Embodiment~\cite{o2024open}               & 2024  & 1.4M & 217 & 64P---720P  & \xmark  & \cmark & \xmark\\
RoboMIND~\cite{wu2024robomind}    & 2024  & 107k & 38 &  & \xmark  & \xmark & \xmark \\
RoboCOIN~\cite{wu2025robocoin}    & 2025  & 180k & 36 &  & \xmark  & \xmark & \xmark \\
Galaxea~\cite{jiang2025galaxea}    & 2025  & 100k & 58 &  & \xmark  & \xmark & \xmark \\
InternData-A1~\cite{tian2025interndata}    & 2025  & 630k & 18 &  & \xmark  & \xmark & \xmark \\
Fourier ActionNet~\cite{fourier2025actionnet}    & 2025  & 13k & 16 & 800P & \xmark  & \xmark & \xmark \\
Humanoid Everyday~\cite{zhao2025humanoid}        & 2025  & 10.3k & 221 & 320P---720P & \xmark  & \xmark & \xmark \\
Agibot World~\cite{bu2025agibot}                 & 2025  & 1M & 87 & 480P & \xmark  & \xmark & \xmark \\
\midrule
\rowcolor{RowRed} \textbf{RoVidX-4M (Ours)}     & 2025  & 4M & 1300+ & 720P & \cmark  & \cmark & \cmark\\
\bottomrule
\end{tabular}
}

\label{tab:magic3m_comparison}
\vspace{-5pt}
\end{table*}



==> tabs/tab_quantitative_analysis.tex <==
%---------------------------------------------Benchmark Table----------------------------------------------------
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{3.8pt}
\caption{\textbf{R-Bench quantitative results.} Evaluations across task-oriented and embodiment-specific dimensions for 18 models from open-source, commercial, and robotics-specific families. The "Avg." column shows the mean score across nine indicators, with task performance in the left block and embodiment performance in the right block. The scores derived from sub-metrics are reported in the Appendix.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{
l c c|
>{\centering\arraybackslash}p{2.1cm} % Manipulation
>{\centering\arraybackslash}p{2.1cm} % Long-horizon
>{\centering\arraybackslash}p{2.1cm} % Multi-entity
>{\centering\arraybackslash}p{2.1cm} % Spatial
>{\centering\arraybackslash}p{2.1cm}|% Reasoning
>{\centering\arraybackslash}p{2.0cm} % Single arm
>{\centering\arraybackslash}p{2.0cm} % Dual arm
>{\centering\arraybackslash}p{2.0cm} % Quad robot
>{\centering\arraybackslash}p{2.0cm}  % Humanoid
}
\toprule
\textbf{Models} & \textbf{Rank} & \textbf{Avg.} &
\multicolumn{5}{c|}{\textbf{Tasks}} &
\multicolumn{4}{c}{\textbf{Embodiments}} \\
 &  &  &
\textbf{Manipulation} & \textbf{Long-horizon} & \textbf{Multi-entity} & \textbf{Spatial} & \textbf{Reasoning} &
\textbf{Single arm} & \textbf{Dual arm} & \textbf{Quad robot} & \textbf{Humanoid} \\
\midrule
\rowcolor{RowRed}
\multicolumn{12}{l}{\textit{Open-source}} \\
Wan2.2\_A14B~\cite{wan2025wan}   & 5  & 0.657 & 0.471 & 0.582 & 0.646 & 0.595 & 0.462 & 0.776 & 0.758 & 0.820 & 0.807 \\
LongCat-Video~\cite{meituanlongcatteam2025longcatvideotechnicalreport} & 8  & 0.598 & 0.522 & 0.547 & 0.547 & 0.420 & 0.252 & 0.729 & 0.738 & 0.819 & 0.810 \\
Wan2.2\_5B~\cite{wan2025wan}     & 10 & 0.554 & 0.444 & 0.502 & 0.548 & 0.477 & 0.315 & 0.556 & 0.637 & 0.746 & 0.766 \\
Wan2.1\_14B~\cite{wan2025wan}    & 11 & 0.548 & 0.433 & 0.473 & 0.555 & 0.385 & 0.276 & 0.588 & 0.679 & 0.740 & 0.804 \\
SkyReels~\cite{chen2025skyreelsv2infinitelengthfilmgenerative} & 12 & 0.533 & 0.361 & 0.408 & 0.503 & 0.472 & 0.293 & 0.622 & 0.686 & 0.758 & 0.698 \\
LTX-Video~\cite{HaCohen2024LTXVideo} & 13 & 0.518 & 0.440 & 0.389 & 0.535 & 0.388 & 0.273 & 0.593 & 0.650 & 0.714 & 0.686 \\
FramePack~\cite{zhang2025framepackv1} & 14 & 0.482 & 0.326 & 0.291 & 0.451 & 0.412 & 0.233 & 0.484 & 0.605 & 0.810 & 0.732 \\
CogVideoX\_5B~\cite{yang2024cogvideox} & 15 & 0.414 & 0.300 & 0.337 & 0.400 & 0.206 & 0.170 & 0.454 & 0.542 & 0.648 & 0.670 \\
HunyuanVideo~\cite{kong2024hunyuanvideo} & 16 & 0.403 & 0.370 & 0.318 & 0.312 & 0.401 & 0.153 & 0.336 & 0.392 & 0.678 & 0.668 \\

\midrule
\rowcolor{RowRed}
\multicolumn{12}{l}{\textit{Commercial}} \\
Wan 2.5~\cite{wan2025wan} & \cellcolor{Top1}1 & 0.725 & 0.544 & \cellcolor{Sub1}0.707 & 0.627 & 0.749 & 0.558 & \cellcolor{Sub1}0.847 & 0.793 & \cellcolor{Sub1}0.891 & 0.819 \\
Hailuo v2~\cite{hailuo2024} & \cellcolor{Top2}2 & 0.723 & \cellcolor{Sub1}0.614 & 0.672 & 0.671 & \cellcolor{Sub1}0.820 & 0.566 & 0.790 & 0.810 & 0.780 & 0.785 \\
Veo 3~\cite{GoogleDeepMind2025Veo3} & \cellcolor{Top3}3 & 0.717 & 0.567 & 0.654 & 0.628 & 0.757 & 0.571 & 0.799 & 0.798 & 0.859 & 0.822 \\
Seedance 1.0~\cite{gao2025seedance} & 4 & 0.712 & 0.575 & 0.638 & \cellcolor{Sub1}0.700 & 0.625 & \cellcolor{Sub1}0.578 & 0.774 & \cellcolor{Sub1}0.832 & 0.848 & \cellcolor{Sub1}0.841 \\
\midrule
\rowcolor{RowRed}
\multicolumn{12}{l}{\textit{Robotics-specific}} \\
Cosmos 2.5~\cite{ali2025world} & 6  & 0.635 & 0.485 & 0.622 & 0.536 & 0.463 & 0.479 & 0.739 & 0.782 & 0.822 & 0.791 \\
DreamGen(gr1)~\cite{jang2025dreamgen} & 7  & 0.604 & 0.429 & 0.484 & 0.577 & 0.583 & 0.339 & 0.744 & 0.766 & 0.760 & 0.760 \\
DreamGen(droid)~\cite{jang2025dreamgen} & 9  & 0.567 & 0.408 & 0.473 & 0.529 & 0.504 & 0.383 & 0.687 & 0.681 & 0.712 & 0.732 \\
UnifoLM-WMA-0~\cite{unifolm-wma-0} & 17 & 0.289 & 0.110 & 0.102 & 0.125 & 0.057 & 0.000 & 0.323 & 0.227 & 0.387 & 0.221 \\
Vidar~\cite{feng2025vidar} & 18 & 0.172 & 0.173 & 0.115 & 0.205 & 0.145 & 0.068 & 0.400 & 0.539 & 0.488 & 0.475 \\
\bottomrule
\end{tabular}

}
\label{tab:magicbench_combined}
\end{table*}
